UniPilot: Enabling GPS-Denied Autonomy Across Embodiments

This paper presents UniPilot, a compact hardware-software autonomy payload that can be integrated across diverse robot embodiments to enable autonomous operation in GPS-denied environments. The system integrates a multi-modal sensing suite including LiDAR, radar, vision, and inertial sensing for robust operation in conditions where uni-modal approaches may fail. UniPilot runs a complete autonomy software comprising multi-modal perception, exploration and inspection path planning, and learning-based navigation policies. The payload provides robust localization, mapping, planning, and safety and control capabilities in a single unit that can be deployed across a wide range of platforms. A large number of experiments are conducted across diverse environments and on a variety of robot platforms to validate the mapping, planning, and safe navigation capabilities enabled by the payload.

==> table/experiment_overview.tex <==
\begin{tabular}{lSSl}
    \toprule
    Sequence    &{Length [\si{\meter}]} &{Maximum Speed [\si{\meter\per\second}]}   &Capabilities\\
    \midrule
    NTNU Elektro  &   &   & State estimation performance in fast flight\\
    NTNU Basement   &   &   & Neural safe navigation policy in clutter\\
    RelyOn  &   &   & Autonomous exploration and inspection\\
    L\o{}kken  &   &    & Autonomous exploration and inspection\\
    Ship Cargo Hold  &   &   & Autonomous exploration and inspection\\
    \bottomrule
\end{tabular}

==> table/software.tex <==
\begin{tabular}{cccc}
    \toprule
    Purpose &Method &Capabilities &Experiments\\
    \midrule
    Control    & & &\\
    Estimation    & & &\\
    Safety    & & &\\
    Planning    & & &\\
     \bottomrule
\end{tabular}
